History-Determinism vs Fair Simulation

An automaton is history-deterministic if its nondeterminism can be resolved on the fly, only using the prefix of the word read so far. This mild form of nondeterminism has attracted particular attention for its applications in synthesis problems. An automaton $A$ is guidable with respect to a class $C$ of automata if it can fairly simulate every automaton in $C$ whose language is contained in that of $A$. In other words, guidable automata are those for which inclusion and simulation coincide, making them particularly interesting for model-checking. We study the connection between these two notions, and specifically the question of when they coincide. For classes of automata on which they do, deciding guidability, an otherwise challenging decision problem, reduces to deciding history-determinism, a problem that is starting to be well-understood for many classes. We provide a selection of sufficient criteria for a class of automata to guarantee the coincidence of the notions, and use them to show that the notions coincide for the most common automata classes, among which are $\omega$-regular automata and many infinite-state automata with safety and reachability acceptance conditions, including vector addition systems with states, one-counter nets, pushdown-, Parikh-, and timed-automata. We also demonstrate that history-determinism and guidability do not always coincide, for example, for the classes of timed automata with a fixed number of clocks.

==> 5cyes-register-timed.tex <==
We apply \cref{cl:Criteria}.\cref{Item:OneTokenGhost} to safety and reachability timed automata.
We begin with the case of register automata.

\begin{proof}[Proof sketch]
The goal is to simulate $\A$ with a delay, as in~\cref{def:Simpleautomata-SigmaShift}.
Registers updates use the current data, so we  duplicate each register and systematically update one copy at each transition; this updated copy becomes ``active'' when the register of $\A$ is updated; if not, it remains passive and gets updated again at the next transition. This guarantees that updates correctly store the previous data value, rather than the current one. The state space remembers which copies of registers are active.
We also store the previous letter in an extra register; then guards operate on this value and the active copies of $\A$'s registers.

From \cite[Lemma 6.3 and Theorem 6.5]{BHLST'23}, $G_1$ characterises history-determinism for safety and reachability LTS, so, from \cref{cl:Criteria}.\cref{Item:OneTokenGhost} we obtain that history-determinism and guidability coincide for safety and reachability register automata.
\end{proof}

For timed automata, we have similar difficulties: delaying a clock reset by a step will affect the value of the clock for future comparisons, and there is no delaying the passage of time. Hence a naive construction would end up recognising the timed language of words in which timestamps are shifted by one. Our $1$-token ghost construction uses similar ideas to the register case: each clock is duplicated, with one copy systematically reset at every transition, in order to simulate retroactive resets. In addition, we can't store timestamps in the way registers can store data, so the state-space stores the effect of the previous delay, by remembering the corresponding region, that is, how the timestamp compares to existing clocks and constants. With this construction, and the $G_1$-characterisation of history-determinism for safety and reachability automata, we obtain the following theorem.

\begin{restatable}{theorem}{cltimedhdguid}\label{cl:timedhd-guid}
For the class of timed automata with safety or reachability acceptance conditions, the notions of history-determinism and guidability coincide.
\end{restatable}

==> App2b-proofofgknotequalsgk+1.tex <==


Given $k\in\PNat$, we construct NFAs $\A_k$ and $\A'_k$, depicted in~\cref{fig:G2vsG3}, over the alphabet $\Sigma = \{1,2,\cdots,k{+}1\}$. In $\A_k$, there is an initial nondeterministic choice, which must guess the third letter of the word. In $\A'_k$, there is a nondeterministic choice from the second state, which must guess a letter that is \textit{not} the third letter. Then, in $G_k(\A',\A)$ Eve wins by choosing a letter that was not guessed in $\A$, as at least one such letter must exist. However, in $G_{k+1}(\A',\A)$ this strategy no longer works since Adam can play on every transition of $\A$ from the initial state and give no information about the third letter.


Formally, we define $\A_k = (\Sigma, P, p_I, \Delta_P,F_P)$, where 
$P = \{p_I\} \cup \{(p,i) \mid i \in [1..k{+}1]\} \cup \{(r,i) \mid i \in [1..k{+}1]\} \cup\{e\}$
is the set of states, $p_I$ is the initial state, and $e$ is the only accepting state.
The transition function $\Delta_P$ consists of the following transitions for each $i \in [1..k{+}1]$:
$p_I \xrightarrow{1} (p,i)$; $(p,i) \xrightarrow{1} (r,i)$; and $(r,i) \xrightarrow{i} e$.

An example of $\A_k$ for $k=2$ is given in \cref{fig:G2vsG3}. Observe that $\A_k$ recognizes the language $1 \cdot 1\cdot \Sigma^{+}$, yet it needs to guess along the first transition what would be the third letter. 

Next, we define $\A'_k = (\Sigma,Q, q_I,\Delta_Q,F_Q)$, where 
$Q = \{q_I,q_1\} \cup \{(s,i) \mid 1\leq i \leq k+1\} \cup\{f\}$ is the set of states, $q_I$ is the initial state, and $f$ is the only accepting state.
The transition function $\Delta_Q$ consists of the following transitions for each $i \in [k+1]$:
$q_I \xrightarrow{1} (q,1)$; $(q,1) \xrightarrow{1} (s,i)$; and $(s,i) \xrightarrow{\Sigma \setminus \{i\}} e$.

An example of $\A'_k$ for $k=2$ is given in \cref{fig:G2vsG3}. %Observe that $\A'_k$ recognizes the same language as $\A_k$, however it needs to guess along the second transition what the third letter would NOT be.
We first show that Eve wins $G_k (\A'_k,\A_k)$:

In the first round, Adam must select the letter 1 (as otherwise he would generate a word not in the language), Eve must select $q_I \xrightarrow{1} (q,1)$ in $\A'_k$, and then Adam selects a transition on each of his $k$ tokens, leading to states $(p,i_1), (p,i_2), \cdots, (p,i_k)$. As $\Sigma = \{1,2, \cdots, k{+}1\}$, there must be some $x \in \Sigma$ that is not equal to any of the $i_j$'s for $j \in [1..k]$. 

In the second round, Adam must select the letter 1 again, Eve chooses the transition $(q,1) \xrightarrow{1} (s,x)$ in $\A'_k$, while Adam's tokens move to $(r,i_1), (r,i_2), (r,i_3) \cdots, (r,i_k)$.

In the third round, Adam must select a letter $y\in \{i_1,i_2, \cdots,i_k\}$ (as otherwise he will not be able to take the next transition), and Eve is able to move her token from $(s,x)$ to the accepting sink state $e$ in $\A'_k$ as $(s,x)$ has transitions to $e$ on all letters apart from $x$. Thus, Eve wins $G_k(\A'_k,\A_k)$.

Next, we show that Adam wins $G_{k+1} (\A'_k,\A_k)$: 
%
In the first round, Adam selects the letter $1$, Eve's token moves deterministically to $(q,1)$, and Adam moves his $k{+}1$ tokens to $(p,1),(p,2), \cdots, (p,k{+}1)$. In the second round, Adam selects the letter $1$ again, and Eve selects some transition $(q,1) \xrightarrow{1} (s,i)$. Adam's tokens move deterministically to $(r,1), (r,2), \cdots, (r,k{+}1)$. In the third round, Adam will select the letter $i$: This causes Eve's run to be rejecting as Eve has no available transition from $(s,i)$ on $i$, while  Adam can move his token at $(r,i)$ to the accepting state $e$. Thus, Adam wins $G_{k+1} (\A'_k,\A_k)$. \qedhere


\begin{figure}
\centering
    \begin{tikzpicture}
		\tikzset{every state/.style = {inner sep=-3pt,minimum size =20}}

        \node (automata) at (0,1) {$\A_2$};
        \node[state] (0) at (0,0) {$p_I$};
		\node[state] (1) at (1.5,1) {$p,1$};
		\node[state] (2) at (1.5,0) {$p,2$};
        \node[state] (3) at (1.5,-1) {$p,3$};
	\node[state] (4) at (3,1) {$r,1$};
        \node[state] (5) at (3,0) {$r,2$};
        \node[state] (6) at (3,-1) {$r,3$};
        \node[state, accepting] (7) at (4.5,0) {$e$};
		\path[-stealth]
		(-.75,0) edge (0)
		(0) edge node[above] {$1$} (1)
		(0) edge node[above] {$1$} (2)
        (0) edge node[above] {$1$} (3)
        (1) edge node[above] {$1$} (4)
        (2) edge node[above] {$1$} (5)
        (3) edge node[above] {$1$} (6)
        (4) edge node[above] {$1$} (7)
        (5) edge node[above] {$2$} (7)
        (6) edge node[above] {$3$} (7)
        (7) edge[loop above] node[right,xshift=0.1cm] {$1,2,3$} ();

        \node (2-token-delay) at (0,-2) {$\A'_2$};
        \node[state] (0a) at (0,-3) {$q_I$};
		\node[state] (2a) at (1.5,-3) {$q,1$};
	\node[state] (4a) at (3,-2) {$s,1$};
        \node[state] (5a) at (3,-3) {$s,2$};
        \node[state] (6a) at (3,-4) {$s,3$};
        \node[state, accepting] (7a) at (4.5,-3) {$f$};
		\path[-stealth]
		(-.75,-3) edge (0a)
		(0a) edge node[above] {$1$} (2a)
        (2a) edge node[above] {$1$} (5a)
        (2a) edge node[above] {$1$} (4a)
        (2a) edge node[above] {$1$} (6a)
        (4a) edge node[above, xshift =0.2cm] {$2,3$} (7a)
        (5a) edge node[above, xshift = -0.05cm, yshift=-0.1cm] {$1,3$} (7a)
        (6a) edge node[below, xshift = 0.2cm] {$1,2$} (7a)
        (7a) edge[loop above] node[right,xshift=0.1cm] {$1,2,3$} ();
    \end{tikzpicture}
    
    \caption{The automata $\A_2$ and $\A'_2$, as per the proof of \cref{cl:Gk+1NotGk}, such that $G_2(\A'_2,\A_2)$, while not $G_3(\A'_2,\A_2)$.}\label{fig:G2vsG3}
   
\end{figure}


==> App2games.tex <==

%\clfromgtog*
%\begin{proof}
%	Let $\strat_1$ and $\strat_{D}$ be strategies witnessing $G_1(\A',\B)$ and $\DSim(\B,\A)$, respectively.
%	We define a strategy $\strat$ for Eve in $\G_{2}(\A',\A)$ by letting her play $\strat_1$ against her imaginary friend Berta, who plays $\strat_{D}$ against Adam's moves. In more detail:
%	In round 0, Adam chooses a letter $\sigma_0$ and Eve responds with the transition sequence $\rho_0=\strat_1(\sigma_0)$.
%	In round $i>0$, 
%	Adam chooses two transition sequences $(\rho^1_{i-1}, \rho^2_{i-1})$ on the letter $\sigma_{i-1}$, and a letter $\sigma_i$, 
%	Berta chooses the transition sequence $\rho^B_{i-1}=\strat_{D}\left( (\rho^1_0,\rho^2_0)\ldots(\rho^1_{i-1},\rho^2_{i-1})\right)$, and then 
%	Eve responds with the transition sequence $\strat_1(\rho^B_{0} \ldots \rho^B_{i-1},\sigma_i)$.
	%
%	Eve's run is as good as Berta's, which is as good as both of Adam's runs, so $\strat$ is a winning strategy in $G_{2}(\A',\A)$.
%\end{proof}

%\clgknotgk*

%\begin{proof}
%	\input{App2b-proofofgknotequalsgk+1}
%\end{proof}



==> App4b-registerautomata.tex <==


We show that safety and reachability register automata are closed under $1$-token ghost. Since the $1$-token game characterises history-determinism for these classes \cite[Lemma 6.3 and Theorem 6.5]{BHLST'23}, we obtain that history-determinism and guidability coincide.

\clsafetyreachabilityregisterautomata*


\newcommand{\prev}{\textit{prev}}
\begin{proof}

The idea of the $1$-token ghost is to copy $\A$ one step behind, as in the $\SigmaShift$  construction (\cref{def:Simpleautomata-SigmaShift}). 
However, since registers can only be updated with the current data, we have to duplicate each register and systematically update one copy or each register at each transition; then this updated copy becomes ``active'' if the next transition updates the said register; if not, it remains passive and gets updated again at the next transition. 
We mark for each register $r$ in the set of registers $R$ which of its two instances is active by augmenting the state space with a function $f:R \rightarrow \{0,1\}$, having that for each register $r$, the $f(r)$ copy is the active one.
We also store the previous letter in an extra register. Guards then operate on the previous letter (stored in its special register) and the active copies of $\A$'s registers. 


More formally, given an RWA $\A=((D,\R),\Sigma_{\bot},Q,\iota,k,\delta,\alpha)$, we define the RWA $\A'=((D,\R),\Sigma_{\bot}, Q',\iota',2k+1,\delta',\alpha')$ as detailed next. Let $R$ be the set of registers of $\A$; we then have in $\A'$ for each $r\in R$  registers $r_{c0}$ and $r_{c1}$ and an additional register $r_\prev$. 
\begin{itemize}
\item $Q'$ consists of pairs $(q,f)$ where $q\in Q$ and $f:R \rightarrow \{0,1\}$, and an initial state $\iota'$.
\item $\delta$ consists of:
\begin{itemize}
\item A transition $\iota'\xrightarrow{\texttt{true}\mid \{r_\prev, r_{c1} \mid r\in R\}}(\iota,f_\iota)$, where $f_\iota(r)=0$ for all $r\in R$, which stores the first letter in $r_\prev$ and in all $1$-copies of registers.
\item For each transition $q\xrightarrow{g\mid s}q'$ of $\A$, a transition $(q,f)\xrightarrow{g'\mid s'}(q',f')$ where $g'$ is as $g$ except that it uses the register $r_{c\,f(r)}$ instead of $r$ and $r_\prev$ instead of the current data; $f'$ updates $f$ so that for all $r\in s$, $f'(r)=1-f(r)$; $s'$ stores the current data in $r_\prev$ and in all registers $r_{c\, 1-f'(r)}$.
\end{itemize}
\item The acceptance condition $\alpha'$ is $\alpha$ projected on the $Q$ component of the state-space, with $\iota'$ being treated identically to $\iota$.
\end{itemize}

We claim that $\A'$ is a $1$-token ghost of $\A$. It recognises $L(\A)$ since there is bijection between configurations of $\A$, paired with the previous data or $\bot$, and configurations of $\A'$. This bijection preserves the $Q$-component of the configuration, and the active copies of $\A$'s registers have the same contents as $\A$'s registers, while $r_\prev$ and the passive registers all contain the previous letter (or $\bot$). This bijection extends to runs of $\A$ and $\A'$, and the states visited along corresponding runs are identical, so the languages of $\A$ and $\A'$ are identical.

Eve's strategy in $G_1(\A',A)$ is to first choose the unique initial transition, and then take the transition corresponding to Adam's choice, via the above mentioned bijection.
%It is straight-forward to build a $1$-token ghost for a register automaton $\A$: it simply stores the last letter in an additional register. Formally, the $1$-ghost $\A'$ of $\A$ has the same states, data domain and registers as $\A$ except that it has an additional register $r$, and $\A'$ can transition from state $q$ with register contents $(r_0,\dots,r_k,r)$ to state $q'$ with register contents $(r_0',\dots,r_k',x)$ over data $x\in \Gamma$, if $\A$ can transition from $q$ with register contents $(r_0,\dots, r_k)$ over data $r$. Furthermore,  from the initial state $\iota$, and initial configuration $(0,\dots,0,0)$, the ghost automaton $\A'$ can transition to $(0,\dots,0,x)$ over each data $x$.

%Then, $\A'$ recognises the same language as $\A$, since the a run of $\A'$ visits the same configurations as a corresponding run of $\A$ over the same word, only one letter later. Furthermore, $G_1(\A',A)$. Indeed, Eve wins this game by first taking the unique transition that stores the first letter in the extra register of $\A$, then copying Adam's transitions in $\A$.

From \cite[Lemma 6.3, Theorem 6.5]{BHLST'23}, $G_1$ characterises history-determinism for safety and reachability automata, so from \cref{cl:Criteria}.\cref{Item:OneTokenGhost} we obtain that history-determinism and guidability coincide for safety and reachability register automata.
\end{proof}

